RemeshingAgent: An Iterative Agent for Repair-Based Decimation of Generated Building Meshes

Aggressively simplifying a generated high-poly building mesh to 0.5-1% of its faces confronts a hard limit. The surface looks complete, yet the mesh is topologically shattered: 10^3-10^4 connected components and non-manifold thin walls. Below a certain budget, every practical decimator "melts": it deletes parts, welds thin walls, or breaks the error tolerance. We attribute this to instance-specific pathology: which components are significant and where the cliff sits vary from mesh to mesh, so no single fixed algorithm suffices, and decimation becomes an iterative loop of cleaning, simplifying, and verifying. We present RemeshingAgent, an agent that turns this loop into a validated process. The melting follows from a triangle-budget decomposition into curvature, crease, component, and genus terms: below the component floor, no output satisfies the repair contract, and cleaning first is the theory-mandated response. At a 0.5% budget the agent stays topology-clean where QEM and vertex clustering melt, matches a commercial remesher on 20 unseen city buildings, and on the 24 training buildings a nine-participant single-workstation blind study prefers our outputs 168:48 (p = 0.0195, subject-level sign test). The trained skill deploys as retrieval replay: 11.7 seconds per mesh on CPU, with no LLM calls.

==> sections/background.tex <==
% background.tex: content merged into theory1.tex (piecewise-smooth defs, already present) and method.tex (mesh representation + operators)


==> sections/discussion.tex <==
% discussion.tex: content merged into conclusion.tex


==> sections/implementation.tex <==
\subsection{Implementation}\label{sec:implementation}

\subsubsection{Agent Architecture}

RemeshingAgent is a layered system. It consists of an OpenAI-compatible LLM client with a ReAct loop and tool executor, a skill layer (registry of mesh-processing skills backed by pymeshlab/MeshLab~\cite{cignoni2008meshlab}, trimesh~\cite{dawson2016trimesh}, and Open3D~\cite{zhou2018open3d}, all CPU-only), an orchestrator with quality-check and topology-optimize sub-agents, and a workflow layer for reporting. The planner prompt has four parts: the system task contract, the current skill document $\skill$, a filter reference card (parameter ranges and failure modes), and a ReAct scratchpad. A stateless LLM has no memory across rounds, so all accumulated knowledge lives in the skill document.

\subsubsection{Skills and Filters}

\emph{optimize\_mesh} exposes pymeshlab methods including planar decimation, QEM, isotropic remeshing, Loop subdivision, tri-to-quad conversion, Taubin smoothing, and \emph{clean\_repair} with two modes, conservative (topological cleanup and degenerate-face removal only) and aggressive (additionally merging close vertices and removing small components by face count and spatial diameter). Mesh repair follows the classical geometric-repair line~\cite{attene2010lightweight}. Table~S7 (supplementary) lists the full skill inventory; the skills central to this paper are \emph{optimize\_mesh}, \emph{execute\_pipeline}, \emph{compute\_metrics}, and \emph{render\_multiview}.

\subsubsection{Training Harness}

The harness (Figure~\ref{fig:algorithm}; pseudocode in the supplementary, S8) processes the training split in rolling groups (one mesh per group, three decimation epochs, then reflect and gate). Per mesh, the current skill is serialized; $B$ candidate pipelines are generated by independent LLM calls; each is executed by the geometry engine; scores and trajectories are saved. Reflection and skill updates run after the whole rollout batch. Every generated pipeline string is hashed and cached; the gate reuses the cache, and a candidate failing on any validation mesh is rejected with the previous best retained.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/fig_algorithm.png}
    \Description{Training loop: forward, score, reflect, apply, and the gate; accepted edits commit to the deployed skill, rejected edits never enter it.}
    \caption{The training loop (cf.\ pseudocode in the supplementary, S8) at group granularity: the gate is the only decision point between candidate and deployed state.}
    \label{fig:algorithm}
\end{figure}

\subsubsection{Reproducibility and Configuration}

Configuration is centralized in the project config module; API credentials are read at runtime from a local credential file (never shipped). One protocol constant matters for interpreting the transfer probe (Section~\ref{sec:exp-transfer}). The retrieval-inference budget is $\max(2000, \text{faces}\times\text{ratio})$, a 2{,}000-face floor that dominates whenever the ratio target falls below it (as it does for every cross-domain mesh, whose 1\% targets range 110--2{,}500). Experiments are deterministic up to LLM sampling temperature and provider availability.


==> sections/method.tex <==
% method.tex: content split into theory1/theory2/theory3 (agent mechanisms embedded after each theorem)


==> sections/theory2.tex <==
% theory2.tex: merged into theory1.tex

